Extended MCDHF calculations of energy levels and transition data for N I

Accurate and extensive atomic data are essential for spectroscopic analyses of stellar atmospheres and other astronomical objects. We present energy levels, lifetimes, and transition probabilities for neutral nitrogen, the sixth most abundant element in the cosmos. The calculations employ the fully relativistic multiconfiguration Dirac-Hartree-Fock and relativistic configuration interaction methods, and span the 103 lowest states up to and including 2s$^2$2p$^2$5s. Our theoretical energies are in excellent agreement with the experimental data, with an average relative difference of 0.07%. In addition, our transition probabilities are in good agreement with available experimental and theoretical data. We further verify the agreement of our data with experimental results via a re-analysis of the solar nitrogen abundance, with the results from the Babushkin and Coulomb gauges consistent to 2% or 0.01 dex. We estimated the uncertainties of the computed transition data based on a statistical analysis of the differences between the transition rates in Babushkin and Coulomb gauges. Out of the 1701 computed electric dipole transitions in this work, 83 (536) are associated with uncertainties less than 5% (10%).

==> tab_energy.tex <==
\startlongtable
\begin{deluxetable*}{lllrrlll}
\tablecaption{\label{tab:energy}Energies (in cm$^{-1}$) and lifetimes (in s ) in both the Babushkin ($\tau_B$) and Coulomb ($\tau_C$) gauges for the lowest 103 levels of \ion{N}{1}.  Energy levels are given relative to the ground state and compared with results from NIST-ASD \citep{NIST_ASD.2021}.
}
\setlength{\tabcolsep}{2.3mm}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{No.} & \colhead{State} & \colhead{$LS$-composition} & \colhead{$E_{RCI} $ }& \colhead{$E_{NIST} $} & \colhead{$\Delta E$} &\colhead{$\tau_B$ }&\colhead{ $\tau_C$ }
}
\startdata
1   & $\mathrm{2s^{2}\,2p^{3}~^{4}S_{3/2}^{\circ}}$            & 0.91                                                                                                                                                & 0           &    0.000       & 0     &             &            \\  
2   & $\mathrm{2s^{2}\,2p^{3}~^{2}D_{5/2}^{\circ}}$            & 0.89                                                                                                                                                & 19426       &    19224.464   & -201  &             &            \\     
3   & $\mathrm{2s^{2}\,2p^{3}~^{2}D_{3/2}^{\circ}}$            & 0.89                                                                                                                                                & 19435       &    19233.177   & -201  &             &            \\     
4   & $\mathrm{2s^{2}\,2p^{3}~^{2}P_{1/2}^{\circ}}$            & 0.85 + 0.03~$\mathrm{2p^{5}~^{2}P^{\circ}}$                                                                                                         & 29142       &    28838.920   & -304  &             &            \\    
5   & $\mathrm{2s^{2}\,2p^{3}~^{2}P_{3/2}^{\circ}}$            & 0.85 + 0.03~$\mathrm{2p^{5}~^{2}P^{\circ}}$                                                                                                         & 29143       &    28839.306   & -303  &             &            \\     
6   & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P_{1/2}}$          & 0.82 + 0.12~$\mathrm{2s\,2p^{4}~^{4}P}$                                                                                                            & 83332       &    83284.070    & -48   &  2.44E-09 &  2.44E-09\\         
7   & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P_{3/2}}$          & 0.82 + 0.12~$\mathrm{2s\,2p^{4}~^{4}P}$                                                                                                            & 83366       &    83317.830    & -48   &  2.42E-09 &  2.42E-09\\         
8   & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P_{5/2}}$          & 0.81 + 0.12~$\mathrm{2s\,2p^{4}~^{4}P}$                                                                                                            & 83413       &    83364.620    & -49   &  2.40E-09 &  2.39E-09\\         
9   & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{2}P_{1/2}}$          & 0.95                                                                                                                                               & 86187       &    86137.350    & -50   &  2.10E-09 &  2.10E-09\\         
10  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{2}P_{3/2}}$          & 0.95                                                                                                                                               & 86270       &    86220.510    & -50   &  2.10E-09 &  2.10E-09\\         
11  & $\mathrm{2s\,2p^{4}~^{4}P_{5/2}}$                         & 0.71 + 0.14~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P}$ + 0.03~$\mathrm{2s\,2p^{3}(^{5}S)\,5p~^{6}P}$                                               & 88213       &    88107.260    &-105   &  7.13E-09 &  6.96E-09\\         
12  & $\mathrm{2s\,2p^{4}~^{4}P_{3/2}}$                         & 0.71 + 0.13~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P}$ + 0.03~$\mathrm{2s\,2p^{3}(^{5}S)\,3p~^{4}P}$                                               & 88257       &    88151.170    &-106   &  6.86E-09 &  6.71E-09\\         
13  & $\mathrm{2s\,2p^{4}~^{4}P_{1/2}}$                         & 0.71 + 0.13~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3s~^{4}P}$ + 0.03~$\mathrm{2s\,2p^{3}(^{5}S)\,5p~^{4}P}$                                               & 88276       &    88170.570    &-106   &  6.72E-09 &  6.58E-09\\         
14  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{2}S_{1/2}^{\circ}}$  & 0.93                                                                                                                                               & 93629       &    93581.550    & -47   &  1.07E-07 &  1.05E-07\\         
15  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}D_{1/2}^{\circ}}$  & 0.94                                                                                                                                               & 94808       &    94770.880    & -37   &  3.99E-08 &  4.03E-08\\         
16  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}D_{3/2}^{\circ}}$  & 0.94                                                                                                                                               & 94830       &    94793.490    & -37   &  3.99E-08 &  4.03E-08\\         
17  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}D_{5/2}^{\circ}}$  & 0.94                                                                                                                                               & 94868       &    94830.890    & -37   &  3.99E-08 &  4.03E-08\\         
18  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}D_{7/2}^{\circ}}$  & 0.95                                                                                                                                               & 94919       &    94881.820    & -37   &  3.98E-08 &  4.03E-08\\ 
19  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}P_{1/2}^{\circ}}$  & 0.95                                                                                                                                               & 95506       &    95475.310    & -30   &  3.34E-08 &  3.40E-08\\         
20  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}P_{3/2}^{\circ}}$  & 0.95                                                                                                                                               & 95524       &    95493.690    & -30   &  3.34E-08 &  3.39E-08\\         
21  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}P_{5/2}^{\circ}}$  & 0.95                                                                                                                                               & 95562       &    95532.150    & -30   &  3.34E-08 &  3.39E-08\\         
22  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{4}S_{3/2}^{\circ}}$  & 0.94                                                                                                                                               & 96791       &    96750.840    & -40   &  2.53E-08 &  2.55E-08\\         
23  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{2}D_{3/2}^{\circ}}$  & 0.92                                                                                                                                               & 96845       &    96787.680    & -58   &  3.89E-08 &  3.89E-08\\         
24  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{2}D_{5/2}^{\circ}}$  & 0.92                                                                                                                                               & 96921       &    96864.050    & -57   &  3.89E-08 &  3.88E-08\\         
25  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{2}P_{1/2}^{\circ}}$  & 0.91                                                                                                                                               & 97842       &    97770.180    & -72   &  3.20E-08 &  3.22E-08\\         
26  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3p~^{2}P_{3/2}^{\circ}}$   & 0.91                                                                                                                                              & 97877       &    97805.840    & -71   &  3.21E-08 &  3.22E-08\\         
27  & $\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3s~^{2}D_{5/2}}$          & 0.94                                                                                                                                               & 99851       &    99663.427   & -187  &  2.57E-09 &  2.58E-09\\         
28  & $\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3s~^{2}D_{3/2}}$          & 0.94                                                                                                                                               & 99851       &    99663.912   & -187  &  2.57E-09 &  2.58E-09\\         
29  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{4}P_{1/2}}$          & 0.94                                                                                                                                               & 103652      &    103622.51   & -29   &  1.19E-08 &  1.21E-08\\         
30  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{4}P_{3/2}}$          & 0.94                                                                                                                                               & 103697      &    103667.16   & -29   &  1.17E-08 &  1.19E-08\\         
31  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{4}P_{5/2}}$          & 0.94                                                                                                                                               & 103765      &    103735.48   & -29   &  1.14E-08 &  1.17E-08\\         
32  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{2}P_{1/2}}$          & 0.91 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}P}$                                                                                             & 104169      &    104144.820   & -24   &  7.47E-09 &  7.68E-09\\         
33  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{2}P_{3/2}}$          & 0.88 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}P}$                                                                                             & 104247      &    104221.630   & -25   &  7.79E-09 &  8.02E-09\\         
34  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}P_{3/2}}$          & 0.86 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{2}P}$                                                                                             & 104646      &    104615.470   & -31   &  9.37E-09 &  9.39E-09\\         
35  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}P_{1/2}}$          & 0.90 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4s~^{2}P}$                                                                                             & 104686      &    104654.030   & -32   &  9.82E-09 &  9.86E-09\\         
36  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F_{3/2}}$          & 0.93                                                                                                                                               & 104697      &    104664.130   & -33   &  2.68E-08 &  2.70E-08\\         
37  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F_{5/2}}$          & 0.91 + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}F}$                                                                                             & 104715      &    104683.060   & -32   &  2.51E-08 &  2.53E-08\\         
38  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F_{7/2}}$          & 0.92 + 0.02~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}F}$                                                                                             & 104749      &    104716.950   & -32   &  2.58E-08 &  2.60E-08\\         
39  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F_{9/2}}$          & 0.96                                                                                                                                               & 104798      &    104765.77   & -32   &  2.77E-08 &  2.80E-08\\  
40  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}F_{5/2}}$          & 0.56 + 0.31~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P}$ + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F}$                                           & 104838      &    104810.360   & -27   &  6.29E-09 &  6.32E-09\\         
41  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P_{5/2}}$          & 0.56 + 0.35~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}F}$ + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D}$                                           & 104849      &    104825.110   & -24   &  5.51E-09 &  5.53E-09\\         
42  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P_{3/2}}$          & 0.86 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D}$                                                                                             & 104882      &    104859.73   & -22   &  4.95E-09 &  4.96E-09\\         
43  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P_{1/2}}$          & 0.90 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D}$                                                                                             & 104908      &    104886.10    & -22   &  4.77E-09 &  4.78E-09\\         
44  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}F_{7/2}}$          & 0.92 + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}F}$                                                                                             & 104910      &    104881.350   & -29   &  7.30E-09 &  7.34E-09\\         
45  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D_{1/2}}$          & 0.91 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P}$                                                                                             & 105006      &    104984.37   & -22   &  2.35E-08 &  2.36E-08\\         
46  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D_{3/2}}$          & 0.88 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P}$                                                                                             & 105018      &    104996.27   & -22   &  2.04E-08 &  2.05E-08\\         
47  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D_{5/2}}$          & 0.89 + 0.05~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}P}$                                                                                             & 105031      &    105008.55   & -22   &  2.19E-08 &  2.20E-08\\         
48  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{4}D_{7/2}}$          & 0.93                                                                                                                                               & 105040      &    105017.600    & -22   &  2.74E-08 &  2.75E-08\\         
49  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}D_{3/2}}$          & 0.94                                                                                                                                               & 105144      &    105119.880   & -24   &  7.58E-09 &  7.57E-09\\         
50  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,3d~^{2}D_{5/2}}$          & 0.94                                                                                                                                               & 105168      &    105143.710   & -24   &  7.53E-09 &  7.52E-09\\  
51  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{2}S_{1/2}^{\circ}}$  & 0.93                                                                                                                                               & 106508      &    106477.800    & -30   &  2.42E-07 &  2.70E-07\\         
52  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}D_{1/2}^{\circ}}$  & 0.94                                                                                                                                               & 106776      &    106758.731  & -17   &  2.36E-07 &  2.50E-07\\         
53  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}D_{3/2}^{\circ}}$  & 0.93                                                                                                                                               & 106795      &    106778.337  & -17   &  2.35E-07 &  2.49E-07\\         
54  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}D_{5/2}^{\circ}}$  & 0.93                                                                                                                                               & 106831      &    106814.459  & -17   &  2.35E-07 &  2.49E-07\\         
55  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}D_{7/2}^{\circ}}$  & 0.95                                                                                                                                               & 106885      &    106868.635  & -17   &  2.36E-07 &  2.51E-07\\         
56  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}P_{1/2}^{\circ}}$  & 0.94                                                                                                                                               & 106996      &    106980.480   & -15   &  1.81E-07 &  1.89E-07\\         
57  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}P_{3/2}^{\circ}}$  & 0.93                                                                                                                                               & 107012      &    106996.032  & -15   &  1.80E-07 &  1.88E-07\\         
58  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}P_{5/2}^{\circ}}$  & 0.93 + 0.02~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}D^{\circ}}$                                                                                     & 107052      &    107037.069  & -15   &  1.81E-07 &  1.89E-07\\         
59  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{2}D_{3/2}^{\circ}}$  & 0.88 + 0.06~$\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3p~^{2}D^{\circ}}$                                                                                     & 107224      &    107182.788  & -42   &  2.28E-07 &  2.28E-07\\         
60  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{2}D_{5/2}^{\circ}}$  & 0.88 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3p~^{2}D^{\circ}}$                                                                                     & 107294      &    107253.106  & -41   &  2.27E-07 &  2.28E-07\\       
61  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{4}S_{3/2}^{\circ}}$  & 0.93                                                                                                                                               & 107494      &    107445.622  & -48   &  1.15E-07 &  1.13E-07\\         
62  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{2}P_{1/2}^{\circ}}$  & 0.90 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3p~^{2}P^{\circ}}$                                                                                     & 107668      &    107588.469  & -79   &  1.39E-07 &  1.43E-07\\         
63  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4p~^{2}P_{3/2}^{\circ}}$  & 0.89 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{1}D)\,3p~^{2}P^{\circ}}$                                                                                     & 107706      &    107628.283  & -78   &  1.40E-07 &  1.43E-07\\         
64  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{4}P_{1/2}}$          & 0.94                                                                                                                                               & 109839      &    109812.233  & -27   &  2.52E-08 &  2.97E-08\\         
65  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{4}P_{3/2}}$          & 0.93                                                                                                                                               & 109884      &    109856.520   & -27   &  2.45E-08 &  2.87E-08\\         
66  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{4}P_{5/2}}$          & 0.94                                                                                                                                               & 109954      &    109926.661  & -27   &  2.32E-08 &  2.69E-08\\         
67  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{2}P_{1/2}}$          & 0.91 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P}$                                                                                             & 110054      &    110035.720   & -18   &  1.29E-08 &  1.80E-08\\         
68  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{2}P_{3/2}}$          & 0.76 + 0.18~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P}$                                                                                             & 110127      &    110103.834  & -23   &  1.59E-08 &  2.23E-08\\         
69  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F_{3/2}}$          & 0.74 + 0.10~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P}$ + 0.05~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{2}P}$                                           & 110218      &    110194.654  & -24   &  5.07E-08 &  5.33E-08\\   
70  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F_{5/2}}$          & 0.78 + 0.09~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F}$ + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$                                           & 110236      &    110212.396  & -24   &  6.14E-08 &  5.94E-08\\     
71  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P_{3/2}}$          & 0.60 + 0.18~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F}$ + 0.14~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{2}P}$                                           & 110243      &    110220.107  & -23   &  2.22E-08 &  2.28E-08\\     
72  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F_{7/2}}$          & 0.83 + 0.07~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$ + 0.06~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F}$                                           & 110271      &    110247.288  & -24   &  7.56E-08 &  7.58E-08\\    
73  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P_{1/2}}$          & 0.82 + 0.08~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$ + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,5s~^{2}P}$                                           & 110272      &    110245.183  & -26   &  2.66E-08 &  2.53E-08\\     
74  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P_{5/2}}$          & 0.43 + 0.25~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F}$ + 0.13~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F}$                                           & 110304      &    110286.305  & -18    &  1.65E-08 &  1.45E-08\\    
75  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F_{5/2}}$          & 0.58 + 0.29~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P}$ + 0.06~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$                                           & 110317      &    110299.974  & -17   &  1.59E-08 &  1.38E-08\\     
76  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F_{9/2}}$          & 0.96                                                                                                                                               & 110328      &    110303.233  & -25   &  9.69E-08 &  1.05E-07\\         
77  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P_{3/2}}$          & 0.54 + 0.34~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$ + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}D}$                                           & 110338      &    110322.721  & -16   &  1.68E-08 &  1.51E-08\\     
78  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D_{5/2}^{\circ}}$  & 0.41 + 0.27~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D^{\circ}}$ + 0.11~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F^{\circ}}$                           & 110365      &    110349.09   & -16   &  6.94E-08 &  6.93E-08\\         
79  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G_{7/2}^{\circ}}$  & 0.35 + 0.24~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G^{\circ}}$ + 0.17~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G^{\circ}}$                           & 110365      &    110349.17   & -16   &  6.98E-08 &  6.98E-08\\         
80  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D_{1/2}}$          & 0.51 + 0.35~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P}$ + 0.09~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P}$                                           & 110366      &    110350.014  & -16    &  2.30E-08 &  2.10E-08\\    
81  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F_{7/2}}$          & 0.78 + 0.10~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F}$ + 0.08~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$                                           & 110381      &    110362.462  & -19   &  2.11E-08 &  1.81E-08\\     
82  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P_{1/2}}$          & 0.58 + 0.36~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D}$                                                                                             & 110401      &    110385.795  & -15   &  1.61E-08 &  1.45E-08\\         
83  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G_{5/2}^{\circ}}$  & 0.48 + 0.37~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D^{\circ}}$ + 0.10~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$                           & 110402      &    110385.29   & -16   &  6.89E-08 &  6.87E-08\\         
84  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D_{7/2}^{\circ}}$  & 0.47 + 0.28~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G^{\circ}}$ + 0.20~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G^{\circ}}$                           & 110402      &    110385.36   & -16   &  6.94E-08 &  6.93E-08\\  
85  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D_{3/2}}$          & 0.56 + 0.38~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P}$                                                                                             & 110410      &    110395.463  & -15   &  2.28E-08 & 2.07E-08\\   
86  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D_{5/2}}$          & 0.74 + 0.18~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}P}$ + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F}$                                           & 110416      &    110401.356  & -15   &  3.79E-08 &  3.53E-08\\    
87  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}D_{7/2}}$          & 0.81 + 0.12~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F}$ + 0.03~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{4}F}$                                           & 110419      &    110403.22   & -15   &  6.16E-08 &  5.82E-08\\    
88  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G_{9/2}^{\circ}}$  & 0.56 + 0.20~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G^{\circ}}$ + 0.19~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F^{\circ}}$                           & 110419      &    110402.09   & -17   &  6.96E-08 &  6.95E-08\\         
89  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G_{7/2}^{\circ}}$  & 0.44 + 0.32~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G^{\circ}}$ + 0.14~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F^{\circ}}$                           & 110419      &    110402.18   & -17   &  6.98E-08 &  6.99E-08\\         
90  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D_{3/2}^{\circ}}$  & 0.33 + 0.32~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D^{\circ}}$ + 0.31~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$                           & 110420      &    110404.50    & -16   &  6.97E-08 &  6.96E-08\\         
91  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D_{5/2}^{\circ}}$  & 0.49 + 0.18~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F^{\circ}}$ + 0.15~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F^{\circ}}$                           & 110420      &    110404.55   & -16   &  7.00E-08 &  7.00E-08\\         
92  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}D_{3/2}}$          & 0.89 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}P}$                                                                                             & 110464      &    110447.032  & -17   &  1.96E-08 &  1.57E-08\\         
93  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D_{3/2}^{\circ}}$  & 0.48 + 0.48~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$                                                                                     & 110475      &    110459.79   & -16   &  6.90E-08 &  6.88E-08\\         
94  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D_{1/2}^{\circ}}$  & 0.96                                                                                                                                               & 110475      &    110459.79   & -16   &  6.93E-08 &  6.91E-08\\         
95  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}D_{5/2}}$          & 0.89 + 0.04~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4d~^{2}F}$                                                                                             & 110486      &    110470.244  & -16   &  1.89E-08 &  1.52E-08\\         
96  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G_{11/2}^{\circ}}$ & 0.96                                                                                                                                               & 110490      &    110473.09   & -17   &  6.90E-08 &  6.88E-08\\         
97  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G_{9/2}^{\circ}}$  & 0.70 + 0.26~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G^{\circ}}$                                                                                     & 110490      &    110473.24   & -17   &  6.97E-08 &  6.97E-08\\         
98  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F_{3/2}^{\circ}}$  & 0.63 + 0.16~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$ + 0.16~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D^{\circ}}$                           & 110502      &    110485.96   & -16   &  7.03E-08 &  7.03E-08\\         
99  & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F_{5/2}^{\circ}}$  & 0.35 + 0.29~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F^{\circ}}$ + 0.26~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$                           & 110502      &    110486.04   & -16   &  7.08E-08 &  7.09E-08\\         
100 & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F_{7/2}^{\circ}}$  & 0.58 + 0.17~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F^{\circ}}$ + 0.14~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}D^{\circ}}$                           & 110514      &    110498.42   & -16   &  7.08E-08 &  7.10E-08\\         
101 & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F_{5/2}^{\circ}}$  & 0.41 + 0.34~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F^{\circ}}$ + 0.11~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}D^{\circ}}$                           & 110514      &    110498.43   & -16   &  7.09E-08 &  7.11E-08\\         
102 & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F_{9/2}^{\circ}}$  & 0.77 + 0.14~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G^{\circ}}$ + 0.05~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}G^{\circ}}$                           & 110518      &    110501.68   & -16   &  7.07E-08 &  7.07E-08\\         
103 & $\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{2}F_{7/2}^{\circ}}$  & 0.59 + 0.17~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}F^{\circ}}$ + 0.11~$\mathrm{2s^{2}\,2p^{2}(^{3}P)\,4f~^{4}G^{\circ}}$                           & 110518      &    110501.83   & -16   &  7.14E-08 &  7.17E-08\\
\enddata
\tablecomments{The third column gives wave function composition (up to three \textit{LS} components with a fractional contribution of $> 0.02$ of the total wave function) in \textit{LS}-coupling. $\Delta E$: the differences ($E_{NIST} - E_{RCI}$) between 
the MCDHF/RCI calculated values and the compiled values from the NIST-ASD. }
\end{deluxetable*}

